On The Round Complexity of Secure Quantum Computation

We construct the first constant-round protocols for secure quantum computation in the two-party (2PQC) and multi-party (MPQC) settings with security against malicious adversaries. Our protocols are in the common random string (CRS) model. - Assuming two-message oblivious transfer (OT), we obtain (i) three-message 2PQC, and (ii) five-round MPQC with only three rounds of online (input-dependent) communication; such OT is known from quantum-hard Learning with Errors (QLWE). - Assuming sub-exponential hardness of QLWE, we obtain (i) three-round 2PQC with two online rounds and (ii) four-round MPQC with two online rounds. - When only one (out of two) parties receives output, we achieve minimal interaction (two messages) from two-message OT; classically, such protocols are known as non-interactive secure computation (NISC), and our result constitutes the first maliciously-secure quantum NISC. Additionally assuming reusable malicious designated-verifier NIZK arguments for NP (MDV-NIZKs), we give the first MDV-NIZK for QMA that only requires one copy of the quantum witness. Finally, we perform a preliminary investigation into two-round secure quantum computation where each party must obtain output. On the negative side, we identify a broad class of simulation strategies that suffice for classical two-round secure computation that are unlikely to work in the quantum setting. Next, as a proof-of-concept, we show that two-round secure quantum computation exists with respect to a quantum oracle.

==> sec-four-round-mpqc.tex <==
\section{Multiparty Quantum Computation in Four Rounds}

We can potentially have a result that any post-quantum $k$-round MPC in the CRS/plain model implies a $k+2$-round MPQC protocol in the CRS/plain model. 
\dakshita{Can we say something similar about the plain model?}

%So given 2-round post-quantum MPC in CRS model, there exists an MPQC that only requires 3 rounds of online communication (it is possible that this is optimal, even 2PC where both parties receive output might require 3 rounds, as noted in BY20). 

Since we have post-quantum constant-round coin tossing, this also implies a constant round MPQC protocol with four rounds of online communication.

Basically, the first round is for exchanging quantum inputs, the second and third round are for computing a particular classical functionality, and the fourth round is for distributing the quantum outputs. 

\begin{itemize}
\item \textbf{Setting.} We have $k$ parties where party 1 is chosen to be the designated party. Each party $i \in [k]$ has an input of $m_i$ qubits, written as $\ket{\psi_{i,1}},\dots,\ket{\psi_{i,m_i}}$. Party 1 will also have some number of ancillary $\ket{0}$ qubits (which function as ``work registers'') as well as ``magic state'' qubits $\ket{T} = T \ket{+}$ qubits to facilitate the computation; for the description of the protocol, these extra qubits will be treated as part of Party 1's input.

The parties wish to jointly compute a quantum circuit $C$, which is assumed to be a ``Clifford + measurement'' circuit which takes standard inputs, ancillary registers, and $\ket{T}$ states. 
\item \textbf{Round 1.} Each party $i \in [k]$:
\begin{itemize}
\item Samples $m_i$ uniformly random $n+1$-qubit Cliffords $E_{i,1},\dots,E_{i,m_i} \leftarrow \mathscr{C}_{\lambda+1}$.
\item For each $j \in [m_i]$, computes $E_{i,j}(\ket{\psi_{i,j}} \otimes \ket{0^\lambda})$, and sends this to party 1; party 1 keeps these qubits to themselves.
\item Generates many EPR pairs, and sends half of each pair to party $i-1$ (where party 0 is taken to be party $k$); this step initializes the $\Pi^{\text{Tel-Enc}}$ input encoding protocol. 
\end{itemize}
\item Before the second round, each party $i \in [k]$ draws a random ``big'' Clifford $F_i \leftarrow \mathscr{C}$. Party 1 concatenates all of its received states $\bigotimes_{i \in [k],j \in [m_i]} E_{i,j}(\ket{\psi_{i,1}} \otimes \ket{0^\lambda})$ along with $\lambda$ additional trap qubits $\ket{0^\lambda}$ \fermi{do we really need $\lambda$ trap qubits for each qubit that we're encrypting?} and applies $V_1$. Each party $i \in [k] \setminus \{1\}$ performs Bell measurements as in the $\Pi^{\text{Tel-Enc}}$ protocol, and the result is that party 1 holds a Quantum One-Time Pad encoding of 
\[F_k \cdots F_1 \left(\left(\bigotimes_{i \in [k],j \in [m_i]} E_{i,j}(\ket{\psi_{i,1}} \otimes \ket{0^\lambda}) \right) \otimes \ket{0^\lambda}\right).\]

\item \textbf{Round 2.} (Round 1 of Classical MPC) The parties send their first round messages for the classical MPC protocol $\mathsf{MPC}(C^{\text{comp}})$, where $C^{\text{comp}}$ is a classical functionality described below. 
\item \textbf{Round 3.} (Round 2 of Classical MPC) The parties send their second round messages for $\mathsf{MPC}(C^{\text{comp}})$.
\item \textbf{Round 4.} Party 1 sends the Clifford encoded outputs and magic states to the corresponding parties. Each party $i \in [k] \setminus \{1\}$ will decrypt using their private Clifford keys, and checks that the trap qubits are $0^\lambda$; if not, they abort.
\end{itemize}

The $C^{\text{comp}}$ functionality works as follows:

% In the first round, each party encodes their inputs with individual Clifford keys and send these encoded inputs to the designated party. They also exchange EPR pairs. 

% Before the second round, each party (including the designated party) draws a random Clifford $V_i$ and performs their Bell measurements. The designated party at this point is teleporting in the states received from every other party, along with the appropriate number of encoded 0 and T states. Now the classical functionality is computed as follows.

%This will be part of the input encoding to be done by the designated party. In the first round, they each send their encoded inputs to the designated party. Also in the first $k$ rounds, they compute a classical MPC that computes the following.

\begin{itemize}
    \item \textbf{Input.} For each $i \in [k]$: party $i$'s Bell measurement results $\vec{a}_i,\vec{b}_i \in \{0,1\}^\ell$, and (classical descriptions of) party $i$'s ``big'' Clifford $F_i$ and its ``small'' Clifford $\{E_{i,j}\}_{j \in [m_i]}$ used to encode individual qubits.
    \item \textbf{Designated Party Output.} Output the appropriate input encoding matrix to the designated party. This will be stripping off the $F_i$, stripping off the Clifford encodings for each input, applying a random linear transformation to the final $2n$ qubits of each $2n+1$ block (in the case of an ancillary 0 input, the linear transformation will be applied to all $2n+1$ qubits, as done in~\cite{EC:DGJMS20}), applying an $X^{r_i}$ to each of the last $n$ qubits of each block, and re-encoding the concatenation of all remaining $n+1$ qubit blocks. Note that this is a Clifford unitary with a classical description, as it is composed entirely of Clifford operations.
    
    Also output an encryption under $\bigoplus_i r_i$ of the Clifford+measurement circuit gadget described in section 4 (including the garbled circuits). This will be slightly modified so that a random subset of the purported magic states prepared and encoded by the designated party are set aside for each party to check later.
    \item \textbf{Non-Designated Party Output.} Output the final Cliffords corresponding to the output qubits and magic states to check to each non-designated party.
\end{itemize}

In the final round, the designated party will send the Clifford encoded outputs and magic states to the corresponding parties, and each will decrypt and check that the trap qubits are 0. Note this strategy does not satisfy unanimous abort, only selective abort, where the adversary can choose a subset of the honest parties to abort while the others may receive the correct output. However, it is guaranteed that if an honest party does not abort, then it recovers the correct output.

Hopefully the view of the designated party after receiving the classical MPC output can be simulated given just the Clifford encoded output qubits. In section 4 there is an outline for simulating the Clifford+measurement circuit gadgets, but we'll also have to handle the input encoding step. Note that instead of responding to the MPC with the correct $r_i$ strings as done in Dulek et al, we are encrypting the MPC's response under the keys $\{r_i\}$, making this non-interactive.

% \subsection{Older stuff}

% We want a primitive that supports the following:
% Client input: $\ket{\psi_1},\dots,\ket{\psi_n}$, quantum circuit $F$
% Server input: nothing

% \begin{itemize}
% \item Client samples a random Clifford $C$ and sends $C(\ket{\psi_1\cdots\psi_n}\otimes 0^n)$ to the server.
% \item Client and Server engage in two-round protocol where at the end of the protocol, the server should send back $C(F(\ket{\psi_1,\dots,\psi_n}),0^{2n-1})$.
% \end{itemize}

% Every party Clifford encodes their own state, and then sends it to the designated party. The designated party runs TelEnc on the concatenation of all the input encoded states. 


% Big Clifford: \url{https://images-na.ssl-images-amazon.com/images/I/61cn0TPm5-L.jpg}

% Steps for the full MPC:
% \begin{itemize}
% \item (First round of quantum communication) Each party sends the EPR pairs to their neighboring parties in order to facilitate the teleportation. Each party also sends their Clifford encoded input.
% \item (classical communication) The MPC sends a small Clifford $C_i$ to each party $i$ (for each $i$, there's actually one $C_i$ for each input bit)
% \item (classical communication) Each party runs the Tel-Enc procedure to obtain $\prod_i C_i(\ket{\psi_i,0^n})$, which is the input encoding of their own input. This involves sending a the Bell-basis measurements to the MPC.
% \item (classical communication) Each party sends their Clifford-encoded input state to the designated party; this happens via teleportation so it's classical communication
% \item (classical communication) The MPC sends a big Clifford $D_i$ to each party. The designated party concatenates all the Clifford-encoded inputs that it gets from all the players, including its own, along with a bunch of states that are supposed to be magic states. Then it appends a bunch of trap qubits.
% \item We run a big Tel-Enc procedure to check that the designated party did this correctly.
% \item At the end of this Tel-Enc procedure, the designated party should have a Clifford encoding of all the input qubits, along with magic states (but this step has not checked that the purported magic states are actually magic states).
% \item Next the designated party receives a classical description of a Clifford+measurement circuit that has the dual purpose of performing magic state distillation, and then applying the entire computation. (every time you do a measurement, you feed the outcome of the measurement into a garbled circuit, which tells you the next clifford to apply)
% \item It sends a classical string to the MPC, and if the classical string checks out, then the result of the computation is accepted. 
% \end{itemize}

==> sec-pq-garble.tex <==
\section{Post-quantum Yao garbled circuit}
\begin{definition}[Post-quantum adaptive security]
\label{def: post-quantum garbling}
A garbling scheme $\textsf{Gb} = (\textsf{GCircuit}, \textsf{GInput})$ for a family of circuits $\mathcal{C}$ is post-quantum adaptively secure if there exist a pair of QPT algorithms $\textsf{Sim} = (\textsf{SimCircuit},\textsf{SimInput})$, such that for any QPT adversary $\mathcal{A}$ the following holds:
$$ \left| \Pr[\textsf{Exp}(1^{\lambda}, \mathcal A, \textsf{Sim}, 0) = 1] -  \Pr[\textsf{Exp}(1^{\lambda}, \mathcal A, \textsf{Sim}, 1) = 1] \right| = negl(\lambda) \,,$$
where the experiment $\textsf{Exp}(1^{\lambda}, A, \textsf{Sim}, b)$ is defined as follows:
\begin{itemize}
    \item[(i)] $\mathcal A$ specifies a circuit $C$ and gets in return $\tilde{C}$ created as follows:
    \begin{itemize}
        \item if $b=0$: $(\tilde{C}, k) \leftarrow \textsf{GCircuit}(1^{\lambda}, C)$
        \item if $b = 1$: $(\tilde{C}, \textsf{state}) \leftarrow \textsf{SimCircuit}(1^{\lambda}, \Phi_{\textsf{topo}}(C))$, where $\Phi_{\textsf{topo}}(C)$ reveals the topology of $C$.
    \end{itemize}
    \item[(ii)] $\mathcal A$ produces a state $\sum_x \alpha_x \ket{x}$, and receives in return:
    \begin{itemize}
        \item if $b=0$: $\sum_x \alpha_x \ket{x} \ket{\textsf{GInput}(k,x)}$
        \item if $b=1$: $\sum_x |\alpha_x|^2 \ket{\textsf{SimInput}(C(x), \textsf{state})}\bra{\textsf{SimInput}(C(x), \textsf{state})}$
    \end{itemize}
    \item[(iii)] $\mathcal A$ outputs a bit $b'$, which is the output of the experiment.  
\end{itemize}
\end{definition}

\begin{theorem} 
If Yao is a \emph{classically} adaptively secure garbling scheme for a family of circuits $\mathcal{C}$, then it is also a \emph{post-quantum} adaptively secure garbling scheme for $\mathcal C$. [currently only holds if PRFs are replaced with random oracles in Yao]
\end{theorem}

\begin{proof}
This is a sketch proof.

Let $\textsf{Gb} = (\textsf{GCircuit}, \textsf{GInput})$ be the Yao garbling scheme. 

To clarify some notation, the garbling key $k$ takes the form $(s^i_{b}: i \in [n], b \in \{0,1\})$. The initial labels $s_b^i$ are the secret keys for PRF based secret key encryptions of the labels in the next layer, and so on.

Let $\mathcal A$ be a quantum adversary as in the security game of Definition \ref{def: post-quantum garbling}.
\vspace{2mm}

The state held by $\mathcal{A}$ just before step (iii) of the security game is the following (I'm omitting auxiliary registers for simplicity; the state in the third register should be a mixed state in general):\fermi{Why does the attacker's state have registers for $C$ and $x$? This doesn't seem right to me since these registers can't be simulated; I would have guessed that the attacker's state is what is written below, but without the $C$ and $x$ registers}
    \begin{equation}
        \mathbb{E}_{\tilde{C},k \leftarrow \textsf{GCircuit}(1^{\lambda}, C)} \ket{C}\bra{C} \otimes \ket{\tilde{C}}\bra{\tilde{C}} \otimes \left((\sum_x \alpha_x \ket{x} \ket{\textsf{GInput}(k,x)})(\sum_x \alpha_x \bra{x} \bra{\textsf{GInput}(k,x)})\right) \,. \label{eq: state 1}
    \end{equation} 
    We will argue that this state is computationally indistinguishable from 
   \begin{equation}
   \mathbb{E}_{\tilde{C},k \leftarrow \textsf{GCircuit}(1^{\lambda}, C)} \ket{C}\bra{C} \otimes \ket{\tilde{C}}\bra{\tilde{C}} \otimes \sum_x |\alpha_x|^2 \ket{x} \ket{\textsf{Ginput}(k,x)}\bra{x}\bra{\textsf{Ginput}(k,x)} \,.
   \label{eq: state 2}
   \end{equation}
Upon substituting Yao's garbling scheme, we have
\begin{equation}
    \eqref{eq: state 1} = \mathbb{E}_{\tilde{C}, s_b^i} \ket{C}\bra{C} \otimes \ket{\tilde{C}}\bra{\tilde{C}} \otimes \left( (\sum_x \alpha_x \ket{x} \ket{s_{x_1}^1, \ldots, s_{x_n}^n}(\sum_x \alpha_x \bra{x} \bra{s_{x_1}^1,\ldots, s_{x_n}^n})\right) \label{eq: state 4}\,,
\end{equation}
and
\begin{equation}
    \eqref{eq: state 2} = \mathbb{E}_{\tilde{C},s_b^i} \ket{C}\bra{C} \otimes \ket{\tilde{C}}\bra{\tilde{C}} \otimes \sum_x |\alpha_x|^2 \ket{x} \ket{s_{x_1}^1, \ldots, s_{x_n}^n}\bra{x} \bra{s_{x_1}^1,\ldots, s_{x_n}^n}  \label{eq: state 5}\,.
\end{equation}

\begin{itemize}
    \item We show that an adversary that distinguishes the states \eqref{eq: state 4} and \eqref{eq: state 5} can be used to construct an adversary that succeeds at the following generic distinguishing task, parametrized by values $\alpha$,$\beta$:
 \begin{itemize}
            \item If $b=0$, the adversary receives \begin{equation}
            \mathbb{E}_{s_0, s_1 \leftarrow \{0,1\}^n}\,\,\, \left(\alpha\ket{0} \ket{s_0} + \beta\ket{1}\ket{s_1}\right)\left(\alpha\bra{0} \bra{s_0} + \beta\bra{1}\bra{s_1}\right)\,. \label{eq: state 12}
            \end{equation}
            together with classical values $H(s_0)$ and $H(s_1)$, for a uniformly random function $H$ with appropriate range, and (superposition) oracle access to $H$.
            \item If $b=1$, the adversary receives \begin{equation}
                \mathbb{E}_{s_0, s_1 \leftarrow \{0,1\}^n}\,\,\,|\alpha|^2\ket{0}\bra{0} \ket{s_0}\bra{s_0} + |\beta|^2\ket{1}\bra{1}\ket{s_1}\bra{s_1}\,. \label{eq: state 13}
            \end{equation}
            together with classical values $H(s_0)$ and $H(s_1)$, for a uniformly random function $H$ with appropriate range, and (superposition) oracle access to $H$.
        \end{itemize}
        To see why this reduction should hold, consider first the case where $x$ is a single bit. The case of arbitrarily long $x$ is obtained by applying the single-bit case result to for each bit of $x$. 
        
        The state that the adversary creates in \eqref{eq: state 4} is 
        $$\mathbb{E}_{\tilde{C}, s_0, s_1 \leftarrow \{0,1\}^n}\,\,\, \ket{C}\bra{C} \otimes \ket{\tilde{C}(s_0, s_1)}\bra{\tilde{C}(s_0,s_1)} \otimes \left(\alpha\ket{0} \ket{s_0} + \beta\ket{1}\ket{s_1}\right)\left(\alpha\bra{0} \bra{s_0} + \beta\bra{1}\bra{s_1}\right)\,. $$
        The only information in $C$ and $\tilde{C}$ that is correlated to the third register are pairs of the form $(r_0, PRF_{s_0}(r_0))$ and $(r_1, PRF_{s_1}(r_1))$ for uniformly random $r$'s (in fact these are not even in the clear in $\tilde{C}$, because they are xored with labels for the successive layer) for random $r_0$ and $r_1$. All the remaining information can be simulated in a reduction. Here, I would have liked to replace the PRFs with random oracles, but I don't quite see that it is possible. I would have liked to reduce to a game in which the adversary sees pairs $(r_0, H(s_0, r_0))$ and $(r_1, H(s_1, r_1))$.
    \item We show that no bounded adversary can succeed at the above distinguishing task (distinguishing \eqref{eq: state 12} and \eqref{eq: state 13}) with non-negligible advantage.
    \begin{itemize}
        \item First replace the random oracle $H$ with a small range distribution i.e. and oracle whose range is a uniformly random exponentially small fraction of the full range, yet still exponentially large. By \cite{zhandry2012construct}, the two oracles are indistinguishable to a bounded-query adversary.
        \item Let $S_0 = H^{-1}(H(s_0))$ and $S_1 = H^{-1}(H(s_1))$. These are exponentially large sets. From the point of view of an unbounded query adversary the challenge is now to distinguish the states:
        \begin{equation}
            \mathbb{E}_{s_0 \leftarrow S_0, s_1 \leftarrow S_1}  \left(\alpha\ket{0} \ket{s_0} + \beta\ket{1}\ket{s_1}\right)\left(\alpha\bra{0} \bra{s_0} + \beta\bra{1}\bra{s_1}\right) \label{eq: state 9}
        \end{equation}
        and 
        \begin{equation}
            \mathbb{E}_{s_0 \leftarrow S_0, s_1 \leftarrow S_1} |\alpha|^2 \ket{0}\bra{0} \ket{s_0}\bra{s_0} + |\beta|^2 \ket{1}\bra{1} \ket{s_1}\bra{s_1}  \label{eq: state 10}
        \end{equation}
     \item One can calculate that states \eqref{eq: state 9} and \eqref{eq: state 10} are negligibly close in trace distance by Lemma \ref{lem: negl trace distance} below. Hence, they are information-theoretically indistinguishable.
    \end{itemize}
    
   \item Finally, using the classical adaptive security of the garbling scheme, we can replace 
   $$ \mathbb{E}_{\tilde{C},k \leftarrow \textsf{GCircuit}(1^{\lambda}, C)} \ket{C}\bra{C} \otimes \ket{\tilde{C}}\bra{\tilde{C}} \otimes \sum_x |\alpha_x|^2 \ket{x} \ket{\textsf{Ginput}(k,x)}\bra{x}\bra{\textsf{Ginput}(k,x)}
   $$
   with $\sum_x |\alpha_x|^2 \ket{\textsf{SimInput}(C(x), \textsf{state})}\bra{\textsf{SimInput}(C(x), \textsf{state})}$.
\end{itemize}

\end{proof}

\begin{lemma}
\label{lem: negl trace distance}
Let $\ket{\psi_0}$ and $\ket{\psi_1}$ be two orthogonal states, and let $\ket{aux_0}$, $\ket{aux_1}$ be two (not necessarily orthogonal) states. Let $S_0, S_1 \subseteq \{0,1\}^n$. Let $\mathcal{S}_0$ and $\mathcal{S}_1$ be distributions over $S_0$ and $S_1$ respectively from now on. Let \fermi{In the following equation, should the $\alpha$ and $\beta$ be $\overline{\alpha}$ and $\overline{\beta}$ in the second parenthesis?}
\begin{equation}
           \rho_0 = \mathbb{E}_{s_0 \leftarrow \mathcal{S}_0, s_1 \leftarrow \mathcal{S}_1} \,\,\, \left(\alpha\ket{\psi_0} \ket{s_0} \ket{aux_0} + \beta\ket{\psi_1}\ket{s_1}\ket{aux_1}\right)\left(\alpha\bra{\psi_0} \bra{s_0}\bra{aux_0} + \beta\bra{\psi_1}\bra{s_1}\bra{aux_1}\right)\,, \label{eq: state 9}
\end{equation}
and 
\begin{equation}
            \rho_1 = \mathbb{E}_{s_0 \leftarrow \mathcal{S}_0, s_1 \leftarrow \mathcal{S}_1} \,\,\,\,|\alpha|^2 \ket{\psi_0}\bra{\psi_0} \otimes \ket{s_0}\bra{s_0} \otimes \ket{aux_0}\bra{aux_0} + |\beta|^2 \ket{\psi_1}\bra{\psi_1} \otimes \ket{s_1}\bra{s_1} \otimes \ket{aux_1}\bra{aux_1} \label{eq: state 10}
\end{equation}
Then 
\begin{equation}
    \|\rho_0-\rho_1\|_1 \leq 2 \cdot 2^{-\frac{\textbf{H}_{min}(\mathcal{S}_0)}{2}} \cdot 2^{-\frac{\textbf{H}_{min}(\mathcal{S}_1)}{2}}\,.
\end{equation}
\end{lemma}
In particular, it is sufficient that one of the two distributions has polynomial min-entropy \fermi{super-logarithmic?} for the trace distance to be negligible.
\begin{proof}
We have
\begin{align}
\| \rho_0 - \rho_1 \| &= \left\| \mathbb{E}_{s_0 \leftarrow \mathcal{S}_0, s_1 \leftarrow \mathcal{S}_1} \left( \alpha \bar{\beta}\ket{\psi_0} \ket{s_0} \ket{aux_0}\bra{\psi_1}\bra{s_1}\bra{aux_1}  +\bar{\alpha}\beta \ket{\psi_1} \ket{s_1} \ket{aux_1}\bra{\psi_0}\bra{s_0}\bra{aux_0} \right) \right\|_1 \\
&\leq |\alpha| |\beta| \left\|\mathbb{E}_{s_0 \leftarrow \mathcal{S}_0, s_1 \leftarrow \mathcal{S}_1}  \ket{\psi_0} \ket{s_0} \ket{aux_0}\bra{\psi_1}\bra{s_1}\bra{aux_1} \right\|_1 \\
&\,\,\,\,+ |\alpha||\beta| \left\|\mathbb{E}_{s_0 \leftarrow \mathcal{S}_0, s_1 \leftarrow \mathcal{S}_1}\ket{\psi_1} \ket{s_1} \ket{aux_1}\bra{\psi_0}\bra{s_0}\bra{aux_0} \right\|_1
\\
&\leq \left\|\mathbb{E}_{s_0 \leftarrow \mathcal{S}_0, s_1 \leftarrow \mathcal{S}_1}  \ket{\psi_0} \ket{s_0} \ket{aux_0}\bra{\psi_1}\bra{s_1}\bra{aux_1} \right\|_1 \\
&\,\,\,\,+ \left\|\mathbb{E}_{s_0 \leftarrow \mathcal{S}_0, s_1 \leftarrow \mathcal{S}_1}\ket{\psi_1} \ket{s_1} \ket{aux_1}\bra{\psi_0}\bra{s_0}\bra{aux_0} \right\|_1 \,. \label{eq: 17}
\end{align}
We upper bound the first summand (the second is a relabelling).
Since the trace norm is invariant under isometries, we replace $\ket{\psi_0}$ and $\ket{\psi_1}$ with $\ket{0}$ and $\ket{1}$ respectively from now on.

We compute the singular values of $\mathbb{E}_{s_0 \leftarrow \mathcal{S}_0, s_1 \leftarrow \mathcal{S}_1}\ket{0}\ket{s_0} \ket{aux_0}\bra{1}\bra{s_1}\bra{aux_1}$ as the square roots of the eigenvalues of \begin{align}
    &\left(\mathbb{E}_{s_0 \leftarrow \mathcal{S}_0, s_1 \leftarrow \mathcal{S}_1} \ket{0}\ket{s_0} \ket{aux_0}\bra{1}\bra{s_1}\bra{aux_1} \right) \left(\mathbb{E}_{s_0' \leftarrow \mathcal{S}_0, s_1' \leftarrow \mathcal{S}_1} \ket{0}\ket{s_0'} \ket{aux_0}\bra{1}\bra{s_1'}\bra{aux_1} \right)^{\dagger} \label{eq: aa}\\
    &= \left(\mathbb{E}_{s_0 \leftarrow \mathcal{S}_0, s_1 \leftarrow \mathcal{S}_1} \ket{0}\ket{s_0} \ket{aux_0}\bra{1}\bra{s_1}\bra{aux_1} \right) \left(\mathbb{E}_{s_0' \leftarrow \mathcal{S}_0, s_1' \leftarrow \mathcal{S}_1}\ket{1}\ket{s_1'} \ket{aux_1}\bra{0}\bra{s_0'}\bra{aux_0} \right) \\
    &= \sum_{s_0, s_0',s_1,s_1'} p_0(s_0)p_0(s_0')p_1(s_1)p_1(s_1') \ket{0}\ket{s_0} \ket{aux_0}\bra{1}\bra{s_1}\bra{aux_1} \,\,\,\ket{1}\ket{s_1'}\ket{aux_1}\bra{0}\bra{s_0'}\bra{aux_0} \label{eq: 18}
\end{align}
where $p_i$ is the probability mass function of $\mathcal{S}_i$. We have
\begin{align}
    \eqref{eq: 18} &= \sum_{s_1} p_1(s_1)^2 \,\,\sum_{s_0, s_0'} p_0(s_0)p_0(s_0') \ket{0}\bra{0} \otimes \ket{s_0}\bra{s_0'} \otimes \ket{aux_0}\bra{aux_0} \\ 
    &= \sum_{s_1} p_1(s_1)^2 \,\, \ket{0}\bra{0} \otimes \left(\sum_{s_0, s_0'} p_0(s_0)p_0(s_0') \ket{s_0}\bra{s_0'} \right) \otimes \ket{aux_0}\bra{aux_0}
\end{align}
Now, notice that \begin{equation}\left(\sum_{s_0, s_0'} p_0(s_0)p_0(s_0') \ket{s_0}\bra{s_0'} \right) =  v v^{\dagger} \,, \label{eq: 23}
\end{equation}
where $v = \sum_{s_0} p_0(s_0) \ket{s_0}$.
In particular, \eqref{eq: 23} has eigenvector $\sum_{s_0} p_0(s_0) \ket{s_0}$ with eigenvalue $\sum_{s_0} p_0(s_0)^2$. We deduce that \eqref{eq: aa} has only one non-zero eigenvalue, namely 
$$ \sum_{s_1} p_1(s_1)^2 \sum_{s_0} p_1(s_0)^2\,.$$
Taking the square root, gives the unique non-zero singular value of $\mathbb{E}_{s_0 \leftarrow \mathcal{S}_0, s_1 \leftarrow \mathcal{S}_1}\ket{0}\ket{s_0} \ket{aux_0}\bra{1}\bra{s_1}\bra{aux_1}$. Finally, notice that
$$ \sum_{s_0} p(s_0)^2 = \mathbb{E}_{s_0 \leftarrow \mathcal{S}_0} \,\,p(s_0) \leq 2^{-\textbf{H}_{min}(\mathcal{S}_0)}\,.$$
Thus, we can upper bound \eqref{eq: 17} by $2 \cdot 2^{-\frac{\textbf{H}_{min}(\mathcal{S}_0)}{2}} \cdot 2^{-\frac{\textbf{H}_{min}(\mathcal{S}_0)}{2}}$, which gives the desired result.


\end{proof}

==> sec-tel-enc.tex <==
\section{Input encoding using teleportation}

We describe an input encoding protocol, which we call $\Pi^{\text{Tel-Enc}}$ that uses teleportation to remove the dependency of the round complexity on the number of players. We will show that $\Pi^{\text{Tel-Enc}}$ securely realizes $\Pi^{\text{Enc}}$, where the latter is the original input encoding protocol from \cite{dulek2020secure}.

\paragraph{Protocol $\Pi^{\text{Tel-Enc}}$.} We describe the protocol for a single input qubit held by party 1. Of course, this can be parallelized for multiple input qubits, as well as for inputs from all parties. We use the same notation as in \cite{dulek2020secure}. In particular we denote by $MT_1T_2$ the input qubit register and trap qubits registers. The protocol is the same as $\Pi^{\text{Enc}}$ except for the following modifications: 
\begin{itemize}
    \item Party $i+1$ prepares $2n+1$ EPR pairs. Sends half of each to party $i$.
    \item After applying the Clifford $F_i$, party $i$ teleports the $2n+1$ qubits of the encoded state to party $i+1$. Let $z_i \in \{0,1\}^{4n+2}$ denote the teleportation measurement outcomes. Party $i$ sends $z_i$ to the MPC. 
    \item Let $\text{Correct}(z_1,\ldots,z_k, F_1,..,F_k)$ be the Pauli correction corresponding to measurement outcomes $z_1\ldots,z_k$ and Cliffords $F_1,\ldots,F_k$. The MPC gives to party 1 a description (as a group element) of the Clifford $V' := V \cdot \text{Correct}(z_1,\ldots,z_k, F_1,\ldots,F_k)$, where $V$ is sampled as in $\Pi^{\text{Enc}}$. 
    \item Party 1 swaps the content of the register in which the teleported state was ``received'' into registers $M T_1 T_2$. Then applies $V'$ to $MT_1T_2$. The rest of the protocol is the same as in $\Pi^{\text{Enc}}$. 
\end{itemize}

We remark that correctness of $\Pi^{\text{Tel-Enc}}$ follows from the definition of $\text{Correct}(z_1,\dots,z_k,F_1,\dots,F_k)$. In particular, the receiving register of party 1 can be written as 
\begin{align*}
(X^{r_k}Z^{s_k})^\dagger F_k \cdots (X^{r_1}Z^{s_1})^\dagger F_1 (\rho \otimes 0^{2k}) &= (X^{r'}Z^{s'})F_k \cdots F_1 (\rho \otimes 0^{2k})
\end{align*}
where for each $i$ we write $z_i = (r_i,s_i)$ for $r_i,s_i \in \{0,1\}^{2n+1}$, and
where $r',s' \in \{0,1\}^{2n+1}$ are determined by $z_1,\dots,z_k,F_1,\dots,F_k$. Since $\text{Correct}(z_1,\dots,z_k,F_1,\dots,F_k) \coloneqq (X^{r'}Z^{s'})^\dagger$, party 1's registers after applying $V'$ are in the form
\[V \cdot F_k \cdots F_1(\rho \otimes 0^{2k}) \]
as in the~\cite{dulek2020secure} input encoding protocol.
\begin{lemma}
$\Pi^{\text{Tel-Enc}}$ securely realizes $\Pi^{\text{Enc}}$.
\end{lemma}

\begin{proof}
We consider two cases.
\paragraph{Case 1: Player 1 is honest (and everyone else is dishonest).} Let $A$ be an adversary for $\Pi^{\text{Tel-Enc}}$. We construct an adversary $A'$ for $\Pi^{\text{Enc}}$ such that the two processes are indistinguishable to any environment. We use the same notation as in \cite{dulek2020secure}: party 1's encoded state is on registers $M$, $T_1$, $T_2$. $R$ is the side-information register of $A$. Additionally, in protocol $\Pi^{\text{Tel-Enc}}$, parties are required to send their teleportation measurement outcomes to the MPC. We denote the registers containing this information by $Z_1,\ldots, Z_k$. We let $W_{1, out}$ and $W_{A, in}$ denote the registers (created by $A$) through which party 1 teleports her encoded state to party 2, and hence to $A$ (when $A$ is honest these registers are initialized with $2n+1$ EPR pairs). In particular, $W_{1, out}$ is a $2n+1$-qubit register. Finally, we let $W_{1, in}$ and $W_{A, out}$ denote the registers through which $A$, acting as party $k$, teleports the state back to party 1 (these registers are initialized honestly by party 1 with $2n+1$ EPR pairs).

We split $A$ into two parts: $A^{(1)}$ which creates a state on registers $W_{1,out}$ and $W_{A, in}$, and, acting as party 2, sends $W_{1, out}$ to party 1; $A^{(2)}$ which performs the rest of the adversary's actions.

$A'$ acts as follows:
\begin{itemize}
    \item $A'$ creates registers $W_{1, out} W_{A, in}$, initialized in the zero state, and runs $A^{(1)}$ on these registers.
    \item $A'$ receives registers $M T_1 T_2$ from party 1. Makes $2n+1$ Bell basis measurements, each involving one of the $2n+1$ qubits in $M T_1 T_2$ and the corresponding qubit in the $2n+1$ qubits of $W_{1, out}$. Stores the outcomes of these measurements as $z_1 \in \{0,1\}^{4n+2}$ in a new register $Z_1$.
    \item $A'$ initializes registers $W_{1, in} W_{A, out}$ with $2n+1$ EPR pairs (across the two registers).
    \item $A'$ initializes registers $Z_2, \ldots Z_k$ (in the zero state). Runs $A^{(2)}$, which acts on registers $W_{A, in}W_{A, out} RZ_2 \ldots Z_k$. Let $\text{Correct}^{W_{1, in} Z_1,\ldots,Z_k}(F_2, \ldots, F_k)$ be the Pauli correction applied on register $W_{1, in}$, based on the values in $Z_1,\ldots,Z_k$ and the sampled Cliffords $F_2,\ldots,F_k$ (notice that the first Clifford $F_1$ is applied before any teleportation errors are incurred, so it doesn't affect the final correction). $A'$ applies $\text{Correct}^{W_{1, in} Z_1,\ldots,Z_k}(F_2, \ldots, F_k)$.
    \item $A'$ swaps the content of register $W_{1,in}$ into register $M T_1 T_2$. Sends the latter registers to party 1.
\end{itemize}

We compute the state of all registers $M T_1 T_2 R$ just before the final measurement of party 1 in protocols $\Pi^{\text{Tel-Enc}}$ and $\Pi^{\text{Enc}}$. In what follows, let $B^{MT_1T_2 W_{1, out} Z_1}$ be a unitary that ``coherently'' performs $2n+1$ Bell basis measurements between registers $M T_1 T_2$ and $W_{1,out}$, ``storing'' outcomes in $Z_1$. Let $\rho^{MR}$ be the state chosen by the environment. 

One can check that in both protocols the overall state just before the final measurement of party 1 is:
\begin{align}
&\mathbb{E}_{E,r,s,F_i} \,\,\textsf{SWAP}^{MT_1T_2,W_{1,in}} V\, \text{Correct}^{W_{1,in}Z_1,\ldots,Z_k}(A^{(2)})^{W_{A, in}W_{A, out} RZ_2 \ldots Z_k} B^{MT_1T_2 W_{1,out} Z_1}(A^{(1)})^{W_{1,out}W_{A, in} R Z_2\ldots Z_k}F_1^{MT_1T_2} \nonumber\\
 &\left(\rho \otimes \ket{0^{2n}}\bra{0^{2n}}^{T_1T_2} \otimes \left(\ket{EPR}\bra{EPR}^{2n+1} \right)^{W_{1,in}W_{A,out}}\otimes \ket{0}\bra{0}^{W_{1,out}W_{A,in}}\right)
F_1^{\dagger} (A^{(1)})^{\dagger}B^{\dagger} (A^{(2)})^{\dagger} \,\text{Correct}^{\dagger} V^{\dagger} \textsf{SWAP}^{\dagger} \,.
\end{align}
As a consequence, the state after party 1's final measurement, including the state of the MPC's memory, is also the same in both protocols.

\paragraph{Case 2: Player 1 is dishonest.} Consider the case with two parties, where party 1 is dishonest and party 2 is honest. Let $A$ be an adversary for $\Pi^{\text{Tel-Enc}}$. We can split $A$ into two parts, $A_1$ and $A_2$. $A_1$ receives the classical string $F_1$ from MPC and acts on registers $MR$ that it receives from the environment, registers $T_1T_2W_{1,in}W_{2,out}$ that are initialized to 0, and register $W_{1,out}$ that is initialized to be one half of a set of EPR pairs, where the other half is in register $W_{2,in}$. After applying its attack unitary, $A_1$ saves registers $RW_{1,in}$ for the next round, measures $MT_1T_2$ in the computational basis to get outcome $z_1$ which it inputs to MPC, and sends register $W_{2,out}$ to party 2. $A_2$ receives $V'$ from MPC, acts on registers $RW_{1,in}$, and swaps $W_{1,in}$ with $MT_1T_2$, to obtain the state of the system $MT_1T_2R$ before the final measurement of party 1.

Now we describe an adversary $A'$ for $\Pi^{\text{Enc}}$, also in two parts. $A'_1$ receives $F_1$ from MPC and registers $MR$ from the environment. It initializes $T_1T_2W_{1,in}W_{2,out}$ to 0 and $W_{1,out}W_{2,in}$ to EPR pairs. Then it runs $A_1$, measures $MT_1T_2$ to obtain the string $z_1$, and applies the Pauli correction defined by $z_1$ to the register $W_{2,in}$. It sends the register $W_{2,in}$ to party 2. $A'_2$ receives a state in registers $MT_1T_2$ from party 2 and $V$ from MPC, where $V = EF_1^\dagger F_2^\dagger$ for some $E$ that includes the new Clifford encoding as well as the random linear transformation. Let $\rho'$ be the state in register $W_{2,in}$ after $A_1$ was applied, and define $\rho \coloneqq F_1^\dagger P_1^\dagger \rho'$, where $P_1$ is the Pauli correction defined by string $z_1$. In $\Pi^{\text{Tel-Enc}}$, the state $F_2P_1F_1\rho$ will be entangled with $W_{2,in}$, and the registers measured to obtain a string $z_2$, which defines a Pauli correction $P_2$. Then $A_2$ will receive $V' = EF_1^\dagger P_1^\dagger F_2^\dagger P_2^\dagger$. However, in $\Pi^{\text{Enc}}$, $A'_2$ will receive the state $F_2F_1\rho$, entangle it with $W_{2,in}$, measure to obtain $z_2$, defining a Pauli $P_2$, and give $V' = VP_2^\dagger = EF_1^\dagger F_2^\dagger P_2^\dagger$ to $A_2$. Then it will run $A_2$ on registers $RW_{1,in}$. This results in the same distribution as in $\Pi^{\text{Tel-Enc}}$ since for any fixed Pauli $P_1$, the distributions $F_2$ and $F_2P_1$ are identical for a uniformly random Clifford $F_2$.



\end{proof}
